Center of circle after perspective transformation

Video-based glint-free eye tracking commonly estimates gaze direction based on the pupil center. The boundary of the pupil is fitted with an ellipse and the euclidean center of the ellipse in the image is taken as the center of the pupil. However, the center of the pupil is generally not mapped to the center of the ellipse by the projective camera transformation. This error resulting from using a point that is not the true center of the pupil directly affects eye tracking accuracy. We investigate the underlying geometric problem of determining the center of a circular object based on its projective image. The main idea is to exploit two concentric circles -- in the application scenario these are the pupil and the iris. We show that it is possible to computed the center and the ratio of the radii from the mapped concentric circles with a direct method that is fast and robust in practice. We evaluate our method on synthetically generated data and find that it improves systematically over using the center of the fitted ellipse. Apart from applications of eye tracking we estimate that our approach will be useful in other tracking applications.

==> arxiv/discussion.tex <==
% !TEX root = main.tex

\section{Discussion and Future Work}

We introduce a simple algorithm to robustly estimate the true center position from a pair of ellipses projected from a pair of concentric circles. We apply our method in the context of eye tracking and use it to find the true pupil center in the image plane. Evaluation based on synthetic data shows promising results, especially comparing to the estimated center of the fitted ellipse. Even though we did not evaluate the performance of the method on the estimation of pupil size, we believe it is possible to estimate the pupil size using the radii ratio. 

Despite the fact that our method can accurately estimate the true pupil center under projective distortion, it does not consider refraction, making it unsuitable for real-world eye tracking applications. However, note that our formulation allows us to estimate the radii ratio of two concentric circles, the pupil and the iris in this case, and the iris boundary is much less affected by the refraction at the corner. Theoretically we could use the estimated ratio to find the exact position of the pupil center as well as the iris center in the camera image. In other words, this would allow us to implicitly model the corner refraction and find the true pupil center under both distortions in the real scenarios. 

Beyond the scope of eye tracking, concentric circles pattern has been commonly used as fiducial markers in computer vision related tasks~\cite{7780436, DeGol_2017_ICCV}. Since detection accuracy and speed are crucial for fiducial marker based real-time application, our method could provide another option for fiducial marker based tracking. We are eager to investigate in this direction in future work.
 
%Magic formula can be directly used in AR calibration for example, we only need a few sparse shapes in space and can then easily estimate the projective transformation of the camera. 





==> arxiv/intro.tex <==
% !TEX root = main.tex


%Over the years, many video-based eye trackers have been used in various studies ranging from perception in Psychology and Cognition to computational modeling and human-computer interaction.
%With recent fast development in virtual reality (VR), video-based eye trackers are commonly integrated in many VR headsets.
%No matter what type of eye trackers is used, the foundation of all valid studies builds on the accuracy of eye tracking. 

It is becoming more and more common to include video cameras in head mounted stereo displays to enable eye tracking in virtual reality environments. In this setting, the optical axis of the eye is usually determined based on the center of the pupil, which can be extracted from the video images. Identification of the pupil in the image stream is commonly done by fitting an ellipse to the boundary between the dark pupil and much lighter iris. This approach introduces two sources of error: 1) the center of the ellipse in the image is not the center of the pupil, because the camera transformation is projective (and not just affine); 2)  the refraction at the cornea distorts the pupil shape in addition to the projective camera transformation. The problems from refraction can be circumvented in other situations by additional tracking equipment~\cite{duchowski2007eye}. Without such equipment it may be possible to compensate the effect based on a computationally involved inverse model~\cite{Dierkes2018}. We focus on the first problem, namely the non-affine mapping of the center. To our knowledge, this is the first work %discussing this source of error and 
providing a computational approach estimating the true pupil center in the context of video-based eye tracking. 

\begin{figure}[t]
    \centering
    \setlength{\unitlength}{0.01\columnwidth}
    \begin{picture}(100,89)(0,0)
        \put(0,-1){\includegraphics[width=\columnwidth]{imgs/annulus.png}}
        \put(22,40){\textsf{\scriptsize(a)}}
        \put(75,40){\textsf{\scriptsize(b)}}
        \put(22,-5){\textsf{\scriptsize(c)}}
        \put(75,-5){\textsf{\scriptsize(d)}}
%        \put(72,18){\(\bp\)}
        \put(81.5,19.5){\(r\)}
        \put(84.5,14){\(R\)}
        \put(27.5,20){\(\bp\)}
        %\graphpaper(0,0)(100,100)
    \end{picture}
    \caption{\label{fig:Teaser}
    A pair of ellipses (a) as the image of a pair of concentric circles (b) in perspective.  Taking the data from a conventional ellipse detection tool (shown in axes in (c)), a simple algorithm proposed in this paper locates the true center \(\bp\) respecting the perspective, and determines the radii ratio \(\nicefrac{R}{r}\) of the inferred circles (d).
    }
\end{figure}


%How to reliably and accurately tracking the pupil position determines the accuracy of eye tracking. Image based pupil detection algorithms are most often used in video-based eye trackers. Pupil boundaries are extracted from eye images and then used to fit an ellipse. The estimated ellipse center is used to infer the actual gaze through a calibration procedure.

% MA: in my understanding the difference between visual and optimal 
%One key challenge is known as the difference between two axes--the visual axis and the optical axis. The visual axis corresponds to the real gaze direction but in video camera what we can observe is only the optical axis. The difference between two axes are caused by the perspective distortion of the video camera and the refraction distortion when light rays are refracted when leaving the eyes. Desktop eye trackers often place additional infrared LEDs next to the video camera and utilize the so-called glint point--the first cornea reflection when light rays are bounced back on the surface of cornea--together with the estimated pupil center to infer the actual gaze point. As the angle between the the visual axis and the optical axis is constant (approximately $5^\circ$ of visual angle~\cite{atchison2000optics}), using both cornear reflection and pupil center together implicitly captures the difference between these two axises. However, glint-based pupil detection faces sever challenges in ourdoor environment, which is targeted by most mobile eye trackers. 

%We introduce a new method to estimate the real center of concentric circles in perspective. We know that a circle can be projective transformed into an ellipse, but the question is does the circle center remain as the ellipse center in the projected plane?

The fact that the center of a circle is not mapped to the center of an ellipse under projective transformations is illustrated in Figure~\ref{fig:Teaser}: The pair of ellipses in (a) is the result of perspectively projecting the two concentric circles in (b) to the image plane. The centers of the two ellipses are not coincident (c), and neither coincides with the projected center $\bp$ of the concentric circles. 
As we explain later, there are in fact many projective transformations that would map a pair of concentric circles to the two ellipses found in the image, however, all of them give rise to the \emph{same} projective center, and also all of them agree on the ratio of the radii. In other words, based on the pair of ellipses, the center of the concentric circles and the ratio of the radii are uniquely determined.
%As we explain later, there are in fact many projective transformations that would map a pair of concentric circles to the two ellipses found in the image, however, all of them give rise to the \emph{same} projective center, and also all of them preserve the ratio of the radii. In other words, while we cannot find the pair of circles based on the pair of ellipses, the center of the concentric circles and the ratio of the radii is uniquely determined.

The set of concentric circles is an instance of a \emph{pencil of conics}. One of the degenerated circles in the group corresponds to the true center and it is invariant under projective transformation. In Section~\ref{sec:MathematicalFoundation} we explain this concept and show how  it leads to a simple formulation for a computational approach.
% In the application setting, this computation leads to a better estimation of the center of the pupil as well as an estimate of the pupil size. 
% compute the true projected center position $\bp$ in the image plane given two ellipses. 

%As a first step towards robust detection of pupil position in glint-free setting, w
We apply our method to estimate the true pupil center by using a pair of ellipses, i.e., the pupil ellipse and the iris ellipse. Tested with synthetic data, we show that our method provides robust estimation of pupil center with respect to projective distortion (see Section~\ref{sec:results}). Compared to the pupil center estimated from ellipse fitting our estimation shows significant improvement, less than one pixel distance to the true pupil center in most cases. 

Apart from eye tracking, our method can also be used for related tasks in computer vision. The idea of exploring the projective invariant properties of concentric circles is not new. It has been used for markers consisting of the two concentric circles specified by a ring ~\cite{1541275} or localization in robotics applications~\cite{6630694}. Compared to the iterative optimization techniques our formulation as an eigenproblem is more direct.
% and is probably computationally more robust and efficient.

%It exploids the fact that cross ratio is invariant under projective transformation. However, its computation relies on iterative optimization, which requires more computational time comparing to our method. Similarly, the pattern of concentric circles has also been used for localization in robotics~\cite{6630694}.

%Most of eye tracking studies use video-based eye tracker, which can be separated in two big categories: desktop stationary eye tracker and mobile eye tracker. Desktop eye tracker is used in lab-controlled experiments, and it offers the best accuracy with the sacrifice of users' movement. On the contrary mobile eye tracker allows users to move freely but with a decreased tracking accuracy. 
%
%In order to be able to estimate where people look, we need to calibrate eye trackers first, which requires a reliable pupil detection for both stationary and mobile eye trackers. In practice, most eye trackers use infrared led to light up iris and the contrast between iris and pupil is higher. This is often called the ``light pupil''. 
%
%There are two known issues related to pupil detection: perspective distortion and refraction distortion caused by iris. When recording the video, eye camera introduces the perspective distortion to the observed image of the eyes. Refraction distortion is caused the different refractive property of cornea. Its large refractive index causes light rays to bend significantly when entering or leaving the eyes. These two types of distortions are the major challenges faced by pupil detection. 
%
%We propose a new but simple formulation of the problem which can potentially deal with both distortions. In this work, we focus on dealing with perspective distortion. Our formulation relies on theorem of relationship between pole and polar line in a complex projective space. We use matrices to represent conics, in our case ellipses and circles, and show that the real projective transformed pupil center can be find through eigen decomposition. Additionally, we could also estimate the ratio between R and r. 
%
%Using synthetic rendering, we show that our algorithm works well. 



==> arxiv/method.tex <==
% !TEX root = main.tex


\section{Concentric Circles in Perspective}
Given an ellipse that is the result of the projective transformation of a circle, is it possible to identify the projected center of the circle?  The answer to this question is no.  There is an infinite set of projective transformations that map a circle to the observed ellipse, while sending the center to an arbitrary points.  Therefore, given only an ellipse from a camera view without any information of the perspective, one cannot retrieve the image of the center of the original  circle.  This center retrieval problem, however, becomes drastically different when the given image contains \emph{two} ellipses coming from a pair of \emph{concentric circles}. In the following we introduce the main observations and the resulting algorithm -- the following section provides the mathematical justification. 

Given two ellipses (or more generally, conics)
% MA: I don't don't think the following statement is true
%on an image plane, one can determine whether they are projective transforms of concentric circles.  If they are, then
there may be many projective transformations that map the ellipses into an inferred pair of concentric circles. Nevertheless, these possible transformations will all agree on
\begin{enumerate}
    \item a unique point \(\bp\) that is sent to the center of the target concentric circles; and
    \item the ratio \(\nicefrac{R}{r}\) of the radius \(R\) of the larger circle to the radius \(r\) of the smaller circle.
\end{enumerate}
In other words, based on only two ellipses in an image, and without any information on the projective transformation from the eye to the image plane of the camera, one can identify the center of the concentric circles in the image and compute the radii ratio of the circles.

It turns out that finding the center point \(\bp\) and the radii ratio only amounts to an eigenvalue problem of a \(3\times 3\) matrix, based on which we give a simple algorithm for the center retrieval problem.

\subsection{Matrix Representation of Conics}
A conic, such as an ellipse, takes a general implicit form
\begin{align}
    \label{eq:ImplicitGeneral}
    Ax^2 + Bxy + Cy^2 + Dx + Ey + F = 0,
\end{align}
which can be expressed in the following matrix form:
\begin{align*}
    \begin{bmatrix}
        x&y&1
    \end{bmatrix}
    \underbrace{\begin{bmatrix}
        A&\nicefrac{B}{2} & \nicefrac{D}{2}\\
        \nicefrac{B}{2} & C & \nicefrac{E}{2}\\
        \nicefrac{D}{2} & \nicefrac{E}{2} & F
    \end{bmatrix}}_{\bQ}
    \begin{bmatrix}
        x\\y\\1
    \end{bmatrix}
    = 0,
\end{align*}
where the symmetric matrix \(\bQ\) is called the matrix representation of the conic, and \(\widetilde\bv = (x,y,1)^\intercal\) is a vector in \emph{homogeneous coordinates}.
Note that the rescaled matrix \(\bQ\mapsto \alpha \bQ\), where \(\alpha\) is a nonzero scalar, defines the same conic. This means the matrix representation is a homogeneous coordinate of the conic. Each conic uniquely corresponds to such a homogeneous matrix representation. 

For an ellipse with geometric parameters \(\bc = (c_x, c_y)\) (geometric centroid), \(a\) (major semiaxis), \(b\) (minor semiaxis) with a rotation angle \(\theta\), the coefficients in \eqref{eq:ImplicitGeneral} are given by
\begin{align*}
    &A = a^2\sin^2\theta + b^2\cos^2\theta,
    &&B = 2(b^2 - a^2)\cos\theta\sin\theta, \\
    &C = a^2\cos^2\theta + b^2\sin^2\theta,
    &&D = -2Ac_x -Bc_y,\\
    &E = -Bc_x -2Cc_y,
    &&F = Ac_x^2 + Bc_xc_y + Cc_y^2 - a^2b^2.
\end{align*}

\subsection{Algorithm}
Let \(\bQ_1, \bQ_2\) be two detected ellipses, represented in matrix form, and assume they are the result of an unknown projective transformation of a pair of concentric circles.  Then the following algorithm finds the center \(\bp\) and the radii ratio \(R/r\) for the inferred pair of concentric circles.
\begin{algorithm}[H]
    \caption{\label{alg:Main}Concentric circles in perspective}
\begin{algorithmic}[1]
\Require \(\bQ_1, \bQ_2\)\Comment Two ellipses as \(3\times 3\) symmetric matrices.
\State\(\bA\coloneqq \bQ_2\bQ_1^{-1}\).
\State\((\lambda_i,\bu_i)_{i=1}^3\gets\) the eigenvalue and eigenvector pairs of \(\bA\), with the observation that \(\lambda_1\approx\lambda_2\) and \(\lambda_3\) distinguished.
\State\(\widetilde\bp = (\widetilde p_x,\widetilde p_y, \widetilde p_z)^\intercal \coloneqq \bQ_1^{-1}\bu_3\).
\State\(\bp \coloneqq (\nicefrac{\widetilde p_x}{\widetilde p_z},\nicefrac{\widetilde p_y}{\widetilde p_z})\).
\Ensure \(\bp\) and \(\nicefrac{R}{r}\coloneqq \sqrt{\nicefrac{\lambda_2\lambda_3}{\lambda_1^2}}\).
\end{algorithmic}
\end{algorithm}

\section{Mathematical Justification}
\label{sec:MathematicalFoundation}
The rather straightforward algorithm \algref{alg:Main} is derived based on projective geometry.  In this section we provide the necessary background about conics in projective planes, and derive the formulae in \algref{alg:Main}.

\subsection{Special Sets of Conics}
In the following we provide a number of basic relations between the algebraic and the geometric aspects of conics.  These notions allow us to characterize projective transforms of concentric circles.
\subsubsection{Degenerate Conics}
A conic, represented as a \(3\times 3\) symmetric matrix \(\bQ\), is \emph{degenerate} if \(\det(\bQ) = 0\).  What this means geometrically is that the conic becomes one point, one line, a union of two lines, or a union of two complex conjugate lines whose intersection is a real point.

\subsubsection{Projective Transformations}
\label{sec:ProjectiveTransformationOfConics}
A projective transformation deforms a conic \(\bQ\) into another conic with matrix \(\bL^{-\intercal}\bQ\bL^{-1}\), where \(\bL\) is some general invertible \(3\times 3\) matrix representing the non-degenerate projective transformation in homogeneous coordinates.

\subsubsection{Intersections of Conics} Two generic conics \(\bQ_1\), \(\bQ_2\) can have four, two, or zero real intersection points.  When the number of intersection points is less than four, what happens is that the missing intersections become imaginary.  If one allows \(x,y\) to be complex, then there are always four intersection points, counted with multiplicity.

\subsubsection{Pencil of Conics}Given two generic conics \(\bQ_1\), \(\bQ_2\), one can construct a family of conics through linear combinations
\begin{align*}
    \bQ_{(\alpha,\beta)} \coloneqq \alpha\bQ_1 +\beta\bQ_2,\quad \alpha,\beta\in\CC.
\end{align*}
This family of conics is called a \emph{pencil of conics}.  Geometrically, the pencil of conics consists of all conics passing through the four fixed (possibly complex) intersection points of \(\bQ_1\) and \(\bQ_2\).  Since a rescaling of the matrix \(\bQ_{(\alpha,\beta)}\) results in the same conic, one may use only one parameter \(\lambda\) replacing \((\alpha,\beta)\) to parametrize the pencil of conics:
\begin{align}
    \label{eq:Pencil}
    \bQ_{(\lambda)}\coloneqq -\lambda\bQ_1 + \bQ_2,\quad\lambda\in\CC.
\end{align}
The minus sign here is for later convenience.

\subsubsection{Circles}A conic \(\bQ\) is a \emph{circle} if \(A = C\) and \(B = 0\) in \eqref{eq:ImplicitGeneral}.  This condition is equivalent to equation \(\widetilde\bv^\intercal\bQ\widetilde\bv = 0\) admitting two special solutions \(\widetilde\bv = (1,i,0)^\intercal\) and \(\widetilde\bv = (1,-i,0)^\intercal\).  The two complex points at infinity  \((1,\pm i, 0)^\intercal\) are called the \emph{circular points}.  (Here, ``point at infinity'' refers to the vanishing 3rd component in the homogeneous coordinate.)

\subsubsection{Concentric Circles}
\label{sec:ConcentricCircles}
 Two conics \(\bQ_1\), \(\bQ_2\) are \emph{concentric circles} if they are not only circles (passing through the circular points \((1,\pm i,0)^\intercal\)) but also that \(\bQ_1\), \(\bQ_2\) intersect \emph{only} at the circular points with multiplicity two.  In other words, \(\bQ_1\), \(\bQ_2\) \emph{touch} at the circular points. The pencil of conics spanned by a pair of concentric circles \(\bQ_1, \bQ_2\) consists of all circles concentric to \(\bQ_1\) and \(\bQ_2\).  In this pencil of concentric circles there are several degenerate conics.  One of them corresponds to the circle collapsed to the center point.  This center point is a degenerate conic as the two complex conjugate lines joining the center point to each circular points.  Another degenerate concentric circle is the single real line connecting the two circular points.

\subsection{Projective Transforms of Concentric Circles}
From \secref{sec:ConcentricCircles} we conclude that two real conics \(\bQ_1\), \(\bQ_2\) can be projectively transformed into a pair of concentric circles if and only if \(\bQ_1\) and \(\bQ_2\) touch at two complex points.  

The statement follows from that under any real projective transformation, the touching points \((1,\pm i,0)^\intercal\) of any pair of concentric circles are transformed to some other pair of complex conjugated points, and at the same time the incidence relations---such as the notion of touching---are preserved.  Conversely, if two real conics touch at two complex points, then these two touching points must be the complex conjugate of each other (since the conics are real).  Hence there exists real projective transformations sending the two touching points to \((1,\pm i,0)^\intercal\).  Such projective transformations effectively map the two conics into a pair of concentric circles. 

\subsubsection{Finding the Center}
Suppose \(\bQ_1\) and \(\bQ_2\) are projective transforms of a pair of concentric circles.  Then finding their common center amounts to seeking a degenerate conic in the pencil of conics spanned by \(\bQ_1\) and \(\bQ_2\).  Using the parametric equation \eqref{eq:Pencil} for the pencil, we solve
\begin{align}
    \label{eq:PreEigenvalueProblem}
    \det\left(-\lambda\bQ_1 + \bQ_2\right) = 0.
\end{align}
Assuming \(\det(\bQ_1)\neq 0\) we rewrite \eqref{eq:PreEigenvalueProblem} as
\begin{align*}
    \det\left(-\lambda\bI + \bQ_2\bQ_1^{-1}\right) = 0,
\end{align*}
which is an eigenvalue problem for
\begin{align*}
    \bA\coloneqq\bQ_2\bQ_1^{-1}.
\end{align*}
The three eigenvalues \(\lambda_1,\lambda_2,\lambda_3\) correspond to three degenerate conics in the pencil.  Two of the degenerate conics coincide (\(\lambda_1=\lambda_2\)), being the the single line joining the two touching points of \(\bQ_1,\bQ_2\). The other distinguished degenerate conic is a real point \(\bp\) (together with two complex conjugate lines) representing the center we look for.

The point \(\bp\) in the degenerate conic \(\bQ_{(\lambda_3)} = -\lambda_3\bQ_1+\bQ_2\) can be found by solving \(\bQ_{(\lambda_3)}\bp = 0\):
\begin{align*}
   & (-\lambda_3\bQ_1+\bQ_2)\bp = 0\quad\implies\quad
   \bA\bQ_1\bp = \lambda_3\bQ_1\bp.
\end{align*}
That is, \(\bp = \bQ_1^{-1}\bu_3\) where \(\bu_3\) is the eigenvector \(\bA\bu_3 =\lambda_3\bu_3\) associated with the eigenvalue \(\lambda_3\).

\subsubsection{Radii Ratio}
A projective transformation (\secref{sec:ProjectiveTransformationOfConics}) \(\bQ_1\mapsto\bL^{-\intercal}\bQ_1\bL^{-1}\), \(\bQ_2\mapsto\bL^{-\intercal}\bQ_2\bL^{-1}\) yields
\begin{align*}
    \bA{}\mapsto{}& (\bL^{-\intercal}\bQ_2\bL^{-1})(\bL^{-\intercal}\bQ_1\bL^{-1})^{-1}\\ 
    &= \bL^{-\intercal} \bQ_2\bQ_1^{-1}\bL^{\intercal} = \bL^{-\intercal}\bA\bL^{\intercal},
\end{align*}
which leaves the eigenvalues of \(\bA\) invariant.  Therefore, the ratios  of eigenvalues \(\lambda_1\colon\lambda_2\colon\lambda_3\) are invariant quantities under projective transformations.  Here we only consider the ratios since the matrices \(\bQ_1\), \(\bQ_2\), \(\bA\) are defined only up to a scale.

For \(\bQ_1\), \(\bQ_2\) that are projective transforms of concentric circles, consider a projective transformation \(\bQ_1' = \bL^{-\intercal}\bQ_1\bL^{-1}\), \(\bQ_2' = \bL^{-\intercal}\bQ_2\bL^{-1}\) so that \(\bQ_1'\) and \(\bQ_2'\) are concentric circles with radii \(r\) and \(R\) respectively.  Since the radii are invariant under translations, we may assume that the concentric circles are centered at the origin without loss of generality.  Then we have
\begin{align*}
    \bQ_1' = 
    \begin{bmatrix}
        1&0&0\\ 0&1&0\\ 0&0&-r^2
    \end{bmatrix},\quad
    \bQ_2' = 
    \begin{bmatrix}
        1&0&0\\ 0&1&0\\ 0&0&-R^2
    \end{bmatrix}
\end{align*}
and
\begin{align*}
    \bA' = \bL^{-\intercal}\bA\bL^{\intercal} = \bQ_2' \bQ_1^{\prime -1} = 
    \begin{bmatrix}
        1 & 0 & 0\\ 0&1&0\\0&0& \nicefrac{R^2}{r^2}
    \end{bmatrix}.
\end{align*}
Thus the invariant eigenvalue ratio of \(\bA\) is given by \(\lambda_1\colon\lambda_2\colon\lambda_3 = 1\colon 1\colon\nicefrac{R^2}{r^2}\).  Therefore, the radii ratio \(\nicefrac{R}{r}\) is encoded in the eigenvalues \(\lambda_1 = \lambda_2, \lambda_3\) of \(\bA\).  

In practice, when the two conics \(\bQ_1, \bQ_2\) are detected with measurement error, the spectrum of \(\bA\) may only have an approximated double \(\lambda_1\approx\lambda_2,\lambda_3\).  In that case we retrieve the radii ratios of the concentric circles by one of the following symmetrizations
\begin{align*}
    \frac{R}{r} \approx \sqrt{\frac{\lambda_2\lambda_3}{\lambda_1^2}}
    \approx \sqrt{\frac{\lambda_1\lambda_3}{\lambda_2^2}} \approx\sqrt{\frac{\lambda_3^2}{\lambda_1\lambda_2}}.
\end{align*}




==> arxiv/preamble.tex <==
% !TEX root = main.tex

% Additional preambles and macros
\usepackage{amssymb}
\usepackage{picinpar,moresize,xfrac,nicefrac,graphpap,dcolumn,wrapfig,graphicx,hyperref}
\microtypesetup{stretch=30,shrink=30}
%\usepackage{parskip}

%\DeclareGraphicsExtensions{.png,.pdf,.jpg}

%\usepackage{showlabels}

%%%%% packages for tikz plots %%%%%
\usepackage{tikz,pgfplots}
\usepgfplotslibrary{colormaps}
\usetikzlibrary{pgfplots.colormaps}
\usepackage{rotating}
\pgfplotsset{compat=newest} 
\pgfplotsset{plot coordinates/math parser=false}
\newlength\figureheight 
\newlength\figurewidth
%%%%% end of tikz packages %%%%%%%%

\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\hypersetup{%
  breaklinks,
  colorlinks=true,
  linkcolor=black,
  anchorcolor=black,
  citecolor=black,
  filecolor=black,
  menucolor=black,
  urlcolor=black,
  bookmarksnumbered,
  pdfencoding=auto,
  pdfstartview=FitH,
  pdfpagemode=UseNone,
  pdfnewwindow=true,
  bookmarksopen=false,
  baseurl={}
}

%recommended additional stuff
\usepackage{soul,array,calc,url,ragged2e,graphpap}
\urlstyle{rm}
\usepackage{booktabs} % better tabular

\usepackage[figure]{hypcap}
\usepackage{mathtools}
\mathtoolsset{centercolon}

% strikethrough machinery
\usepackage[normalem]{ulem}
\usepackage{cancel}
%end of package loading

% double brackets
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother
%end double brackets


\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\defref}[1]{Def.~\ref{#1}}
\newcommand{\teqref}[1]{Eq.~(\ref{#1})}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\appref}[1]{App.~\ref{#1}}
\newcommand{\thmref}[1]{Thm.~\ref{#1}}
\newcommand{\lemref}[1]{Lem.~\ref{#1}}
\renewcommand{\algref}[1]{Alg.~\ref{#1}}


%% for pseudocode
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\Proc}[1]{\mbox{\textsc{#1}}}
\renewcommand{\algorithmicforall}{\textbf{for each}}
\renewcommand{\algorithmicrepeat}{\textbf{do}}
\renewcommand{\algorithmicuntil}{\textbf{while}}
\let\ForEach\ForAll
\let\Do\Repeat
\let\dWhile\Until

% MACRO
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\newcommand{\one}{\mathbbold{1}}
\usepackage{xfrac,nicefrac}


\def\ZZ{\mathbb{Z}}
\def\RR{\mathbb{R}}
\def\NN{\mathbb{N}}
\def\SS{\mathbb{S}}
\def\PP{\mathbb{P}}
\def\HH{\mathbb{H}}
\def\CC{\mathbb{C}}
\def\JJ{\mathbb{J}}
\def\CP{\mathbb{CP}}
\def\RP{\mathbb{RP}}
\def\HP{\mathbb{HP}}
\def\TM{T\!M}
\def\TN{T\!N}
\def\TL{T\!L}
\def\TQ{T\!Q}
\def\bA{\mathbf{A}}
\def\bI{\mathbf{I}}
\def\bL{\mathbf{L}}
\def\bQ{\mathbf{Q}}
\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bff{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bp{\mathbf{p}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bS{\mathbf{s}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\br{\mathbf{r}}
\def\btr{\mathbf{\tilde{r}}}
\def\bn{\mathbf{n}}
\def\bt{\mathbf{t}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\ip{\,\iota}
\def\ext{\mathrm{ext}}
\def\inclusion{\,j}
\def\diff{\,d}
\def\codiff{\diff^\dagger}
\def\id{\mathrm{id}}

\def\blambda{\boldsymbol{\lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bsigma{\boldsymbol{\sigma}}
\def\boldzero{\mathbf{0}}

%\def\varDelta{\vartriangle\!\!}
\def\varDelta{\Deltait}

\def\sE{\mathscr{E}}
\def\sH{\mathscr{H}}
\def\sM{\mathscr{M}}
\def\sS{\mathscr{S}}

\def\nn{\mathbbm{n}}
\def\tt{\mathbbm{t}}

\def\frakg{\mathfrak{g}}
\def\frakh{\mathfrak{h}}
\def\frakt{\mathfrak{t}}

\def\Ham{\mathrm{Ham}}
\def\Symp{\mathrm{Symp}}
\def\frakham{\mathfrak{ham}}
\def\fraksymp{\mathfrak{symp}}


\DeclareMathOperator*{\argmin}{argmin}



\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\im}{Im}
%\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\atan}{atan2}
\DeclareMathOperator{\spanset}{Span}
\DeclareMathOperator{\imag}{im}
\DeclareMathOperator{\length}{Length}
\DeclareMathOperator{\area}{Area}
\DeclareMathOperator{\vol}{Vol}
\DeclareMathOperator{\hel}{Hel}
\DeclareMathOperator{\cp}{cp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\tr}{tr}

\def\Euler{\mathrm{Euler}}
\def\ISF{\mathrm{ISF}}
\def\LL{\mathrm{LL}}
\def\Dirichlet{\mathrm{D}}

\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand*{\conj}[1]{\overbar{#1}}

\newcommand{\idx}[1]{{\mathsf{#1}}}

\newcommand{\lk}{\mathop{\mathrm{lk}}\nolimits}

\newcommand{\grad}{\mathop{\mathrm{grad}}\nolimits}
\newcommand{\sgrad}{\mathop{\mathrm{sgrad}}\nolimits}
\newcommand{\curl}{\mathop{\mathrm{curl}}\nolimits}
\renewcommand{\div}{\mathop{\mathrm{div}}\nolimits}
\newcommand{\LD}{\mathop{\mathscr{L}}\nolimits}
\newcommand{\hess}{\mathop{\mathrm{Hess}}\nolimits}

\newcommand{\ppt}{\tfrac{\partial}{\partial t}}


%%%%%%% COMMENTS
\newcommand{\XW}[1]{{\bf\textcolor[rgb]{0.2,0.7,0.3}{XW: #1}}}
\newcommand{\AC}[1]{{\bf\textcolor[rgb]{0.2,0.5,0.8}{AC: #1}}}
\newcommand{\MA}[1]{{\bf\textcolor[rgb]{0.8,0.5,0.2}{MA: #1}}}

==> arxiv/related.tex <==
% !TEX root = main.tex

\section{Background and Related Work}

%Video-based eye tracking estimates gaze direction based on mainly two measurements--the pupil center and the corner reflection point~\cite{duchowski2007eye}. The corner reflection point is the first cornea reflection when light rays are bounced back on the surface of cornea, and it is also called the glint. Most often pupil appear dark in camera images as under common lighting conditions, but in special eye tracking system pupil could also appear bright under external infrared light sources~\cite{holmqvist2011eye}. Nowadays dark-pupil system is commonly used in eye tracking systems. The estimation of the pupil center is based on image analysis algorithms where the boundary of the pupil is fitted with an ellipse and the euclidean center of the ellipse is taken as the pupil center~\cite{Swirski2012, Fuhl2016}. The corner reflection point center can be estimated similarly as it appears as a bright spot in the camera image. The estimated pupil center and the corner reflection are then mapped to gaze position in a target space through calibration. However, in most mobile eye tracking system, only the estimated pupil center is used for calibration~\cite{Kassner2014}. As cornea detection becomes challenging in outdoor environment, mobile eye trackers rely on glint-free eye tracking system.

The estimation of gaze direction in video-based eye tracking relies on measuring the pupil center~\cite{duchowski2007eye, holmqvist2011eye}.  Image analysis algorithms are used to estimate the pupil center. The boundary of the pupil is fitted into an ellipse, and its euclidean center is taken as the pupil center~\cite{Swirski2012, Fuhl2016}. The estimated pupil center is then mapped to gaze direction through calibration, very often with the aid of glint, known as the corner reflection, reflected from a controlled light source. However, most mobile eye tracking system are based on glint-free tracking systems~\cite{Kassner2014}. 

 
How to accurately estimate pupil center position is of major concern in the eye tracking community. The main challenges are risen from distortions in the captured images, namely the projective distortion and the refractive distortion~\cite{4564194, Dierkes2018}. Projective distortion moves the projected pupil center away from the ellipse center as shown in Figure~\ref{fig:Teaser}. The refractive distortion is caused by the different refractive index of cornea ($n=1.33$, $n_{air}=1.0$~\cite{atchison2000optics}), which leads to irregularly distorted pupil boundaries in the camera image. Such distortion depends on the camera viewing direction~\cite{Fedtke10} even when the cornea surface is simplified to a perfect sphere. The analysis gets more complicated when the curvature of the cornea changes~\cite{barsingerhorn2017optics}. Glint-based eye tracking systems implicitly model the refraction distortion~\cite{1634506}, for example by using the difference vector between pupil center and corner reflection for gaze estimation. 

Apart from the above described feature-based gaze estimation, appearance-based gaze estimation methods rely on the detection of eye features in the images~\cite{Mora2014, Park2018}, such as the iris center and the eye corners. These methods aim to track the eye movements for example with webcams. Image resolution in the eye region is limited and the appearances of pupil and cornea are less distinguishable. Very often full faces are visible in the images, therefore, facial landmarks are used as additional information in deep learning methods~\cite{Palmero2018RecurrentCF, Zhang2019}. However, simultaneous detection of both pupil and iris is difficult in both feature-based methods and appearance-based methods, and it inevitably requires many empirical parameter settings~\cite{Yeong2013, szczepanski2014pupil}. Robust detection of both pupil and iris remains as a challenging problem, especially that irises are partially occluded by eyelids. 

Additionally, model-based gaze estimations have been proposed where multiple eye images are used to optimize a three-dimensional eye ball model~\cite{Swirski2013}. Recently a model-fitting approach accounting for cornea refraction has been proposed~\cite{Dierkes2018}. In principle, these model fitting methods are based on ray tracing, which is a considerably expensive procedure. It results in a non-linear minimization problem which requires iterative solving procedures.  

We propose a simple method utilizing the underlying geometric properties of two concentric circles, the pupil and the iris. Our method directly computes the true pupil center in the camera image as well as the projective invariant radii ratio. In general, large distance to the camera image center leads to large projective distortion. In the context of eye tracking, this means larger pupils are more seriously distorted. Recent study~\cite{HOOGE20191} shows that changes in pupil sizes can lead to sever accuracy drops in eye tracking. Pupil size has been used to study observer's mental cognitive load~\cite{Palinko2010} as well as fatigues when using VR headsets~\cite{UKAI2008106}. Our method can also be used to accurately estimate the pupil size (in these applications). 
%As iris boundaries suffer less from the refractive distortion, together with the radii ratio from our method, we can easily compute the radius of pupil.

%We approach the problem by respecting the invariances in projective geometry, and obtain precise estimation of the projected pupil center position, which allows more subtle measurement. 



==> arxiv/results.tex <==
% !TEX root = main.tex

\section{Results}
\label{sec:results}

We apply our method to estimate the true pupil center using the pupil ellipse and the iris ellipse and evaluate it on synthetic data. 

\subsection{Experimental Setup}

Synthetic eye images are rendered using the 3D model proposed in~\cite{Swirski2014} with cornea refractive index set to be 1.0 (see Figure~\ref{fig:ps} for examples). The true projected pupil center in the camera image is directly computed from the 3D model, and we also compute the pupil ellipse and the iris ellipse in the image plane. The pupil center estimated by our method is compared to 1) the Euclidean center of the pupil ellipse in the image plane and 2) the pupil center estimated by image based ellipse fitting following the method proposed in~\cite{Swirski2012}.

Eye camera is placed $3$ cm in front of the eye, similar to the camera position in a mobile eye tracker. We experiment with various viewing angles (rotations of the camera), and three different pupil sizes when the eyes fixate at various targets. Fixation targets are evenly sampled from a circle that is placed perpendicular to the ground. We compare the Euclidean distance in pixel unit between the true pupil center in the image plane and the estimated pupil center using different methods. 

\subsection{Camera Rotation}

With a fixed distance to the eye, the camera is placed at a set of locations that are possible in practice. We use spherical coordinates to describe the rotations. Polar angle $\phi$ defines the rotation angle between the camera and the horizontal plane, and azimuthal angle $\theta$ describes the camera rotation in the horizontal plane. 

\begin{figure}[!t]
    \setlength{\unitlength}{0.01\columnwidth}
    \begin{picture}(100,70)(0,0)
        \put(0,38){\includegraphics[width=.49\columnwidth]{imgs/camera_near_10.pdf}}
        \put(21,35){\textsf{\scriptsize(a)}}
        \put(50,38){\includegraphics[width=.49\columnwidth]{imgs/camera_near_20.pdf}}
        \put(71,35){\textsf{\scriptsize(b)}}
        \put(0,-2){\includegraphics[width=.49\columnwidth]{imgs/camera_near_30.pdf}}
        \put(22,-5){\textsf{\scriptsize(c)}}
        \put(50,-2){\includegraphics[width=.49\columnwidth]{imgs/camera_near_40.pdf}}
        \put(71,-5){\textsf{\scriptsize(d)}}
    \end{picture}
\caption{Estimation errors in different camera positions. $x$ axis corresponds to rotation angle $\theta$ in degree and $y$ axis is the estimation error measured in pixels. From (a) to (d), rotation angle $\phi$ changes from $10^\circ$ to $40^\circ$. In each plot, $\theta$ varies from $30^\circ$ to $70^\circ$.}
\label{fig:cam}
\end{figure}

Figure~\ref{fig:cam} shows the estimation errors using different methods. We test with $\phi$ varying from $10^\circ$ to $40^\circ$ and $\theta$ varies from $30^\circ$ to $70^\circ$. In all tested scenarios, our method gives the best estimation with less than one pixel distance to the true pupil center. Estimated Euclidean centers of the pupil ellipse deviate away from the true pupil center. Image based ellipse fitting gives better estimation as more sample points from the boundary detection are used for ellipse fitting. However, the fitting fails when $\theta$ is large. In such cases, the projected pupil is small in the camera image, subsequently with less camera distortion. Therefore, the estimated pupil positions get closer to its true position. As shown in Figure~\ref{fig:cam}, estimation errors decreases with an increasing $\theta$ from left to right in each plot. 

\subsection{Pupil Size}

As we see from previous test, the estimation accuracy of the Euclidean ellipse center is correlated to the pupil size in the image plane. In this second experiment, we experiment with three different pupil sizes and compare the estimations when the eyes look at different targets. We evenly place 36 targets on a circle that lies perpendicular to the ground. Figure~\ref{fig:ps} shows the results where estimation error measured in pixel is the y-axis and x-axis corresponds to the rotation angle of the eye measured in degree. As expected, large pupil size leads to large estimation error. All estimation methods get worse but our method consistently provides the most accurate estimation. Once again, image based ellipse fitting method fails when the eyes are tilted to some extend as shown by the second image in each plot. 

\begin{figure*}[!t]
    \setlength{\unitlength}{0.01\columnwidth}
    \begin{picture}(100,44)(0,0)
	 \put(0,-3){\includegraphics[width=.33\textwidth]{imgs/rotation_sp.pdf}}
	 \put(10, 31){\includegraphics[width=0.15\columnwidth]{imgs/rotation_sp_0}}
	 \put(25, 21){\includegraphics[width=0.15\columnwidth]{imgs/rotation_sp_15}}
	 \put(70,-3){\includegraphics[width=.33\textwidth]{imgs/rotation.pdf}}
	 \put(80, 31){\includegraphics[width=0.15\columnwidth]{imgs/rotation_0}}
	 \put(95, 21){\includegraphics[width=0.15\columnwidth]{imgs/rotation_15}}
	 \put(140,-3){\includegraphics[width=.33\textwidth]{imgs/rotation_lp.pdf}}
	 \put(150, 31){\includegraphics[width=0.15\columnwidth]{imgs/rotation_lp_0}}
	 \put(165, 21){\includegraphics[width=0.15\columnwidth]{imgs/rotation_lp_15}}
    \end{picture}
\caption{Estimation errors with various pupil size. Camera is placed at a fixed position in front of the eye while fixation targets are evenly sampled from a circle in front. Pupil size increases from left to right and embedded eye images show examples when the eyes are rotated to the left and right. $x$ axis corresponds to rotation angle of the eyes in degree and $y$ axis is the estimation error measured in pixels.}
\label{fig:ps}
\end{figure*}

%\subsection{Error with refraction}

